Certification for mu-calculus with winning strategies

We define memory-efficient certificates for $\mu$-calculus model checking problems based on the well-known correspondence of the $\mu$-calculus model checking with winning certain parity games. Winning strategies can independently checked, in low polynomial time, by observing that there is no reachable strongly connected component in the graph of the parity game whose largest priority is odd. Winning strategies are computed by fixpoint iteration following the naive semantics of $\mu$-calculus. We instrument the usual fixpoint iteration of $\mu$-calculus model checking so that it produces evidence in the form of a winning strategy; these winning strategies can be computed in polynomial time in $|S|$ and in space $O(|S|^2 |{\phi}|^2)$, where $|S|$ is the size of the state space and $|\phi|$ the length of the formula $\phi$\@. The main technical contribution here is the notion and algebra of partial winning strategies. On the technical level our work can be seen as a new, simpler, and immediate constructive proof of the correspondence between $\mu$-calculus and parity games.

==> conclusion.tex <==
{\bf TBD}

==> related_work.tex <==
There have been many results and algorithms for constructing witnesses and counterexamples of
various forms for different sublogics, including $\mathit{LTL}$, $\mathit{ACTL}$,  $\mathit{CTL}$, $\mathit{CTL}^*$,  
of the $\mu$ calculus~\cite{clarke1995efficient,bierezhuclarke1999,peled2001falsification,tancleaveland2002,clarke2002tree,shankarsorea2003,gurfinkel2003proof}\@. 
Here, however, we restrict our comparison to research results on witness generation for the full $\mu$ calculus.

Local model checking procedures for determining whether finite-state systems have properties expressible in the $\mu$ calculus incrementally construct tableau proof~\cite{winskel1989local,stirling1989local,cleaveland1990tableau}, which can be 
proof-checked independently. However the size of the constructed tableau can be exponential in the number of states 
of the model. Based on the tableau method of local $\mu$ calculus model checking, Kick~\cite{kick1995generation}
proposes an optimized construction of witnessing tableau proofs based on identifying isomorphic subproofs.
Namjoshi~\cite{namjoshi2001certifying} introduced the notion of {\em certifying model checker} that can generate
independently checkable witnesses for properties verified by a model checker. He defines witnesses for properties of
labelled transition systems expressed in the $\mu$ calculus based on parity games over alternating tree automata.
His technical developments rely on $\mu$ calculus signatures~\cite{streettemerson94} for termination,
and exploits the correspondence between $\mu$-calculus model checking with winning parity 
games~\cite{emerson1991tree}\@. In contrast to the above methods, the witnesses generated by our global 
model checking algorithm is rather small, namely quadratic in the size of the state space. 




% Emerson, Jutla, Sistla (1993)  On model checking for fragments of mu-calculus, CAV 1993 
% Sorea: Dubious witnesses and spurious counterexamples 
